Remember the Past: Distilling Datasets into Addressable Memories for Neural Networks

We propose an algorithm that compresses the critical information of a large dataset into compact addressable memories. These memories can then be recalled to quickly re-train a neural network and recover the performance (instead of storing and re-training on the full original dataset). Building upon the dataset distillation framework, we make a key observation that a shared common representation allows for more efficient and effective distillation. Concretely, we learn a set of bases (aka ``memories'') which are shared between classes and combined through learned flexible addressing functions to generate a diverse set of training examples. This leads to several benefits: 1) the size of compressed data does not necessarily grow linearly with the number of classes; 2) an overall higher compression rate with more effective distillation is achieved; and 3) more generalized queries are allowed beyond recalling the original classes. We demonstrate state-of-the-art results on the dataset distillation task across six benchmarks, including up to 16.5% and 9.7% in retained accuracy improvement when distilling CIFAR10 and CIFAR100 respectively. We then leverage our framework to perform continual learning, achieving state-of-the-art results on four benchmarks, with 23.2% accuracy improvement on MANY. The code is released on our project webpage https://github.com/princetonvisualai/RememberThePast-DatasetDistillation.

==> sections/SVHN_compressors.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{figures/Compressors_all.pdf}
   \caption{Visualization of learned compressors. Top row: compressors learned on SVHN, from left to right are digit classes from $1$ to $10$. Middle row: CIFAR10 results with classes Plane, Car, Bird, Cat, Deer, Dog, Frog, Horse, Ship and Truck. Bottom row: 16 compressors learned as basis on CIFAR10. For top row and middle row, compressor has size $32\times 32\times 3$, while the bottom row has size $16\times 16\times 3$. Shapes of objects are emerging in the compressors, especially on class-specific compressors of SVHN and CIFAR10.}
   \label{fig:visualization}
\end{figure}


==> sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} Details are in main paper and more in the supplementary materials.
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} More details are in the supplementary materials.
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> tables/table_bptt_gm.tex <==
\begin{table}[t]
\begin{center}
\begin{tabular}{lccc}
\toprule
 & Steps & w/o moment. & w/ moment. \\
\hline
\hline
 \multirow{5}{*}{CIFAR10} 
 & 1 & 29.4${\pm}$0.9 & - \\
 
 & 10 & 33.4${\pm}$0.7 & \textbf{40.4${\pm}$0.6} \\
 
 & 20 & 36.0${\pm}$0.4 & \textbf{44.8${\pm}$0.9} \\
 
 & 50 & 38.4${\pm}$0.4 & \textbf{46.2${\pm}$0.7} \\
 
 & 100 & 38.0${\pm}$0.4 & \textbf{47.2${\pm}$0.8} \\
 
 \hline
 \multirow{5}{*}{SVHN}
 
  & 1 & 28.8${\pm}$0.1 & -  \\
 
 & 10 & 42.7${\pm}$1.4 & \textbf{54.6${\pm}$2.0} \\
 
 & 20 & 50.5${\pm}$1.7 & \textbf{64.2${\pm}$1.7} \\
 
 & 50 & 52.4${\pm}$2.3 & \textbf{69.4${\pm}$1.0} \\
 
 & 100 & 52.4${\pm}$1.4 & \textbf{70.1${\pm}$1.1} \\
\bottomrule
\end{tabular}
\end{center}
\caption{}\label{tbl:moment}
\end{table}

==> tables/table_cl2.tex <==
\begin{table}[t]
\small
\begin{center}
\begin{tabular}{lccc}
\toprule
 Methods & RA & BTI \\
 \hline
 HAT &  72.06 & -0.00 \\
 
 ER-Res &  71.73 & -0.06 \\
 
 A-GEM & 63.98 & -0.15 \\
 
 GPM & 72.48 & -0.00 \\
 \hline

 Ours & \textbf{73.29} & - \\
 
\bottomrule
\end{tabular}
\end{center}
\caption{CIFAR-100.}\label{tbl:cl2}
\end{table}

==> tables/table_cl_main_backup.tex <==
\begin{table*}[h]
\begin{center}
\scalebox{0.8}{

\begin{tabular}{lccccccccr}
\toprule
  & \multicolumn{2}{c}{Rotations} & \multicolumn{2}{c}{Permutations}  & \multicolumn{2}{c}{MANY} & \multicolumn{2}{c}{CIFAR-100}\\
 \cmidrule(lr){2-3}
 \cmidrule(lr){4-5}
 \cmidrule(lr){6-7}
 \cmidrule(lr){8-9}
  & RA & BTI & RA & BTI & RA & BTI & RA & BTI \\
  \hline
 \textsc{Online}  & 53.38$^{\pm1.53}$ & -5.44$^{\pm1.70}$ & 55.42$^{\pm0.65}$ & -13.76$^{\pm1.19}$ & 32.62$^{\pm0.43}$ & -19.06$^{\pm0.86}$ & 32.62$^{\pm0.43}$ & -19.06$^{\pm0.86}$   \\
 EWC     &  57.96$^{\pm1.33}$ & -20.42$^{\pm1.60}$ & 62.32$^{\pm1.34}$ & -13.32$^{\pm2.24}$ & 33.10$^{\pm0.14}$ & -18.50$^{\pm0.91}$ \\
 GEM     & 67.38$^{\pm1.75}$ & -18.02$^{\pm1.99}$ & 55.42$^{\pm1.10}$ & -24.42$^{\pm1.10}$ & 39.50$^{\pm0.62}$ & -17.50$^{\pm0.41}$  \\
 MER     & 77.42$^{\pm0.78}$ & -5.60$^{\pm0.70}$ & 73.46$^{\pm0.45}$ & -9.96$^{\pm0.45}$ & 51.00$^{\pm0.54}$ & -13.57$^{\pm0.45}$  \\
 C-M  & 77.33$^{\pm0.29}$ & -7.88$^{\pm0.05}$ & 74.54$^{\pm0.54}$ & -10.36$^{\pm0.14}$ & 51.33$^{\pm0.52}$ & -16.57$^{\pm0.65}$  \\
 Sync    & 74.07$^{\pm0.58}$ & -6.66$^{\pm0.44}$ & 70.54$^{\pm1.54}$ & -14.02$^{\pm2.14}$ & 47.93$^{\pm0.59}$ & -18.50$^{\pm0.71}$ \\
 La-M & 77.42$^{\pm0.65}$ & -8.64$^{\pm0.40}$ & 74.34$^{\pm0.67}$ &-7.60$^{\pm0.51}$& 50.43$^{\pm0.21}$& -10.00$^{\pm0.36}$ \\
 sp-LaM  & 77.77$^{\pm0.58}$ & -8.16$^{\pm0.61}$ & 76.88$^{\pm0.72}$ & -8.39$^{\pm0.63}$ & 50.81$^{\pm0.79}$ & -13.73$^{\pm0.73}$ \\
 \hline
 Ours  & \textbf{80.32$^{\pm\textbf{0.28}}$}  & - & \textbf{78.48$^{\pm\textbf{0.76}}$} & - & \textbf{74.07$^{\pm\textbf{0.51}}$} & - \\
\bottomrule
\end{tabular}

}
\end{center}
\caption{We show that ``compress-then-recall" is a strong baseline that outperforms state-of-the-art methods on the three benchmarks MNIST Rotations, Permutations and MANY. Baseline numbers are from ~\cite{gupta2020maml} or obtained from public official repos.}\label{tbl:cl}
\end{table*}


==> tables/table_main_withbptt.tex <==
\begin{table*}[t]
\begin{center}
\small
\begin{tabular}{lccccccccccc}
\toprule
 & I/C & DC & DSA & KIP (NN) & CAFE$^*$ & TM & DM &Ours$^{\text{BPTT}}$ & Ours \\
\hline
\hline
\multirow{3}{*}{MNIST} & 1 & 91.7$\pm$0.5 & 88.7$\pm$0.6 & 90.1$\pm$0.1 & 93.1${\pm}$0.3 & - & 89.7$\pm$0.6  & 95.2$\pm$0.3 & \textbf{98.7$\pm$0.7} \\

& 10 & 97.4$\pm$0.2 & 97.8$\pm$0.1 & 97.5$\pm$0.0 & 97.5${\pm}$0.1 & - & 97.5$\pm$0.1  & 98.8$\pm$0.1 & \textbf{99.3$\pm$0.5} \\

& 50 & 98.8$\pm$0.2 & 99.2$\pm$0.1 & 98.3$\pm$0.1 & 98.9${\pm}$0.2 & - & 98.6$\pm$0.1 & 99.2$\pm$0.1 & \textbf{99.4$\pm$0.4} \\
\hline
\multirow{3}{*}{F-MNIST} & 1 & 70.5$\pm$0.6 & 70.6${\pm}$0.6 & 73.5${\pm}$0.5 & 77.1${\pm}$0.9 & - & - & 83.9$\pm$0.4 & \textbf{88.5$\pm$0.1} \\

& 10 &  82.3$\pm$0.4 & 84.6${\pm}$0.3 & 86.8${\pm}$0.1 & 83.0${\pm}$0.3 & - & - & 89.1$\pm$0.2 &  \textbf{90.0$\pm$0.7} \\

& 50 & 83.6$\pm$0.4 & 88.7${\pm}$0.2 & 88.0${\pm}$0.1 & 88.2${\pm}$0.3 & - & - & 90.4$\pm$0.1 & \textbf{91.2$\pm$0.3} \\
\hline
\multirow{3}{*}{SVHN} & 1 & 31.2${\pm}$1.4 & 27.5${\pm}$1.4 & 57.3${\pm}$0.1 & 42.9${\pm}$3.0 & - & - & 71.6${\pm}$0.8 & \textbf{87.3${\pm}$0.1} \\

& 10 &  76.1${\pm}$0.6 & 79.2${\pm}$0.5 & 75.0${\pm}$0.1 & 77.9${\pm}$0.6 & - & - & 83.1${\pm}$0.3 & \textbf{89.1${\pm}$0.2} \\

& 50 & 82.3${\pm}$0.3 & 84.4${\pm}$0.4 & 80.5${\pm}$0.1 & 82.3${\pm}$0.4 & - & - & 86.5$\pm$0.2 & \textbf{89.5$\pm$0.2} \\
\hline
\multirow{3}{*}{CIFAR10} & 1 & 28.3${\pm}$0.5 & 28.8${\pm}$0.7 & 49.9${\pm}$0.2 & 31.6${\pm}$0.8 & 46.3${\pm}$0.8 & 26.0${\pm}$0.8 & 49.1$\pm$0.6 & \textbf{66.4$\pm$0.4} \\

& 10 & 44.9${\pm}$0.5 & 52.1${\pm}$0.5 & 62.7${\pm}$0.3 & 50.9${\pm}$0.5  & 65.3${\pm}$0.7& 48.9${\pm}$0.6 & 62.4$\pm$0.4 & \textbf{71.2$\pm$0.4} \\

& 50 &  53.9${\pm}$0.5 & 60.6${\pm}$0.5 & 68.6${\pm}$0.2 & 62.3${\pm}$0.4 & 71.6${\pm}$0.2 & 63.0${\pm}$0.4 & 70.5$\pm$0.4 & \textbf{73.6$\pm$0.5} \\
\hline
\multirow{2}{*}{CIFAR100} & 1 & 12.8${\pm}$0.3 & 13.9${\pm}$0.3 & 15.7${\pm}$0.2 & 14.0${\pm}$0.3 & 24.3${\pm}$0.3 & 11.4${\pm}$0.3 & 21.3${\pm}$0.6 & \textbf{34.0${\pm}$0.4} \\

& 10 & 25.2${\pm}$0.3 & 32.3${\pm}$0.3 & 28.3${\pm}$0.1 & 31.5${\pm}$0.2  & 40.1${\pm}$0.4 & 29.7${\pm}$0.3 & 34.7${\pm}$0.5 & \textbf{42.9${\pm}$0.7} \\
\bottomrule
\end{tabular}
\end{center}
\caption{We compare our method with previous works on ConvNet performance recovery. Our algorithm consistently outperforms all previous methods and achieves state-of-the-art. $^*$Note that we selected the best results from CAFE and CAFE + DSA. 
}\label{tbl:main}
\end{table*}


==> tables/table_momentum.tex <==
\begin{table}[t]
\begin{center}
\small
\begin{tabular}{lccc}
\toprule
 & Steps & w/o moment. & w/ moment. \\
\hline
\hline
 \multirow{5}{*}{CIFAR10} 
 & 1 & 29.4${\pm}$0.9 & - \\
 
 & 10 & 33.4${\pm}$0.7 & \textbf{40.4${\pm}$0.6} \\
 
 & 20 & 36.0${\pm}$0.4 & \textbf{44.8${\pm}$0.9} \\
 
 & 50 & 38.4${\pm}$0.4 & \textbf{46.2${\pm}$0.7} \\
 
 & 100 & 38.0${\pm}$0.4 & \textbf{47.2${\pm}$0.8} \\
 
 \hline
 \multirow{5}{*}{SVHN}
 
  & 1 & 28.8${\pm}$0.1 & -  \\
 
 & 10 & 42.7${\pm}$1.4 & \textbf{54.6${\pm}$2.0} \\
 
 & 20 & 50.5${\pm}$1.7 & \textbf{64.2${\pm}$1.7} \\
 
 & 50 & 52.4${\pm}$2.3 & \textbf{69.4${\pm}$1.0} \\
 
 & 100 & 52.4${\pm}$1.4 & \textbf{70.1${\pm}$1.1} \\
\bottomrule
\end{tabular}
\end{center}
\caption{Long unrolls and momentum term improves performance.}\label{tbl:bptt}
\end{table}

==> tables/table_syn_cls.tex <==
\begin{wraptable}{r}{4cm}
%\begin{table}[t]
\small
\begin{center}
\begin{tabular}{lcccc}
\toprule
 Storage & 2-way & 5-way \\
 \hline
 1 I/C & 72.53 & 46.45 \\
 
 10 I/C & 75.37 & 48.60 \\
 
 \hline
 
 Real & 92.23 & 82.72 \\
\bottomrule
\end{tabular}
\end{center}
\caption{CIFAR100 disjoint.}\label{tbl:syn_cls}
\vspace{-3mm}
%\end{table}
\end{wraptable}
